Microlensing of the broad emission lines in 27 gravitationally lensed quasars. Broad line region structure and kinematics

We aim to study the structure and kinematics of the broad line region (BLR) of a sample of 27 gravitationally lensed quasars with up to five different epochs of observation. This sample is composed of ~100 spectra from the literature plus 22 unpublished spectra of 11 systems. We measure the magnitude differences in the broad emission line (BEL) wings and statistically model the distribution of microlensing magnifications to determine a maximum likelihood estimate for the sizes of the C IV, C III], and Mg II emitting regions. The BELs in lensed quasars are expected to be magnified differently owing to the different sizes of the regions from which they originate. Focusing on the most common BELs in our spectra (C IV, C III], and Mg II), we find that the low-ionization line Mg II is only weakly affected by microlensing. In contrast, the high-ionization line C IV shows strong microlensing in some cases, indicating that its emission region is more compact. Thus, the BEL profiles are deformed differently depending on the geometry and kinematics of the corresponding emitting region. We detect microlensing in either the blue or the red wing (or in both wings with different amplitudes) of C IV in more than 50% of the systems and find outstanding asymmetries in the wings of QSO 0957+561, SDSS J1004+4112, SDSS J1206+4332, and SDSS J1339+1310. This observation indicates that the BLR is, in general, not spherically symmetric and supports the existence of two regions in the BLR, one insensitive to microlensing and another that only shows up when it is magnified by microlensing.

==> bib_paper.tex <==
@ARTICLE{Wang2020,
       author = {{Wang}, Shu and {Shen}, Yue and {Jiang}, Linhua and {Grier}, C.~J. and
         {Horne}, Keith and {Homayouni}, Y. and {Peterson}, B.~M. and
         {Trump}, Jonathan R. and {Brandt}, W.~N. and {Hall}, P.~B. and
         {Ho}, Luis C. and {Li}, Jennifer I-Hsiu and {Hernand
        ez Santisteban}, J.~V. and {Kinemuchi}, K. and {McGreer}, Ian D. and
         {Schneider}, D.~P.},
        title = "{The Sloan Digital Sky Survey Reverberation Mapping Project: How Broad Emission Line Widths Change When Luminosity Changes}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jun,
          eid = {arXiv:2006.06178},
        pages = {arXiv:2006.06178},
archivePrefix = {arXiv},
       eprint = {2006.06178},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv200606178W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Homayouni2020,
       author = {{Homayouni}, Y. and {Trump}, Jonathan R. and {Grier}, C.~J. and
         {Horne}, Keith and {Shen}, Yue and {Brandt}, W.~N. and
         {Dawson}, Kyle S. and {Alvarez}, Gloria Fonseca and {Green}, Paul J. and
         {Hall}, P.~B. and {Hern{\'a}ndez Santisteban}, Juan V. and
         {Ho}, Luis C. and {Kinemuchi}, Karen and {Kochanek}, C.~S. and
         {Li}, Jennifer I. -Hsiu and {Peterson}, B.~M. and {Schneider}, D.~P. and
         {Starkey}, D.~A. and {Bizyaev}, Dmitry and {Pan}, Kaike and
         {Oravetz}, Daniel and {Simmons}, Audrey},
        title = "{The Sloan Digital Sky Survey Reverberation Mapping Project: Mg II Lag Results from Four Years of Monitoring}",
      journal = {\apj},
     keywords = {Active galaxies, Galaxy nuclei, Quasars, Active galactic nuclei, 17, 609, 1319, 16, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = sep,
       volume = {901},
       number = {1},
          eid = {55},
        pages = {55},
          doi = {10.3847/1538-4357/ababa9},
archivePrefix = {arXiv},
       eprint = {2005.03663},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...901...55H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Braibant2014,
       author = {{Braibant}, L. and {Hutsem{\'e}kers}, D. and {Sluse}, D. and
         {Anguita}, T. and {Garc{\'\i}a-Vergara}, C.~J.},
        title = "{Microlensing of the broad-line region in the quadruply imaged quasar HE0435-1223}",
      journal = {\aap},
     keywords = {gravitational lensing: micro, galaxies: active, quasars: emission lines, quasars: individual: HE0435-1223, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = may,
       volume = {565},
          eid = {L11},
        pages = {L11},
          doi = {10.1051/0004-6361/201423633},
archivePrefix = {arXiv},
       eprint = {1405.5014},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...565L..11B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Clavel1991,
       author = {{Clavel}, J. and {Reichert}, G.~A. and {Alloin}, D. and
         {Crenshaw}, D.~M. and {Kriss}, G. and {Krolik}, J.~H. and
         {Malkan}, M.~A. and {Netzer}, H. and {Peterson}, B.~M. and
         {Wamsteker}, W. and {Altamore}, A. and {Baribaud}, T. and {Barr}, P. and
         {Beck}, S. and {Binette}, L. and {Bromage}, G.~E. and {Brosch}, N. and
         {Diaz}, A.~I. and {Filippenko}, A.~V. and {Fricke}, K. and
         {Gaskell}, C.~M. and {Giommi}, P. and {Glass}, I.~S. and
         {Gondhalekar}, P. and {Hackney}, R.~L. and {Halpern}, J.~P. and
         {Hutter}, D.~J. and {Joersaeter}, S. and {Kinney}, A.~L. and
         {Kollatschny}, W. and {Koratkar}, A. and {Korista}, K.~T. and
         {Laor}, A. and {Lasota}, J. -P. and {Leibowitz}, E. and {Maoz}, D. and
         {Martin}, P.~G. and {Mazeh}, T. and {Meurs}, E.~J.~A. and
         {Nair}, A.~D. and {O'Brien}, P. and {Pelat}, D. and {Perez}, E. and
         {Perola}, G.~C. and {Ptak}, R.~L. and {Rodriguez-Pascual}, P. and
         {Rosenblatt}, E.~I. and {Sadun}, A.~C. and {Santos-Lleo}, M. and
         {Shaw}, R.~A. and {Smith}, P.~S. and {Stirpe}, G.~M. and {Stoner}, R. and
         {Sun}, W.~H. and {Ulrich}, M. -H. and {van Groningen}, E. and
         {Zheng}, W.},
        title = "{Steps toward Determination of the Size and Structure of the Broad-Line Region in Active Galactic Nuclei. I. an 8 Month Campaign of Monitoring NGC 5548 with IUE}",
      journal = {\apj},
     keywords = {Active Galactic Nuclei, Astronomical Spectroscopy, Galactic Structure, Iue, Seyfert Galaxies, Emission Spectra, Time Series Analysis, Ultraviolet Spectra, Variability, Astrophysics, GALAXIES: INDIVIDUAL NGC NUMBER: NGC 5548, GALAXIES: NUCLEI, GALAXIES: SEYFERT, ULTRAVIOLET: SPECTRA},
         year = 1991,
        month = jan,
       volume = {366},
        pages = {64},
          doi = {10.1086/169540},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1991ApJ...366...64C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Motta2017,
   author = {{Motta}, V. and {Mediavilla}, E. and {Rojas}, K. and {Falco}, E.~E. and 
	{Jim{\'e}nez-Vicente}, J. and {Mu{\~n}oz}, J.~A.},
    title = "{Probing the Broad-Line Region and the Accretion Disk in the Lensed Quasars HE 0435-1223, WFI 2033-4723, and HE 2149-2745 Using Gravitational Microlensing}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1703.00400},
 keywords = {gravitational lensing: strong, quasars: emission lines, quasars: individual: HE 0435-1223, WFI 2033-4723, HE 2149-2745},
     year = 2017,
    month = feb,
   volume = 835,
      eid = {132},
    pages = {132},
      doi = {10.3847/1538-4357/835/2/132},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...835..132M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Fian2018,
   author = {{Fian}, C. and {Guerras}, E. and {Mediavilla}, E. and {Jim{\'e}nez-Vicente}, J. and 
	{Mu{\~n}oz}, J.~A. and {Falco}, E.~E. and {Motta}, V. and {Hanslmeier}, A.
	},
    title = "{Microlensing and Intrinsic Variability of the Broad Emission Lines of Lensed Quasars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1805.09619},
 keywords = {gravitational lensing: micro, quasars: emission lines, quasars: general },
     year = 2018,
    month = may,
   volume = 859,
      eid = {50},
    pages = {50},
      doi = {10.3847/1538-4357/aabc0d},
   adsurl = {http://adsabs.harvard.edu/abs/2018ApJ...859...50F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Fian2016,
   author = {{Fian}, C. and {Mediavilla}, E. and {Hanslmeier}, A. and {Oscoz}, A. and 
	{Serra-Ricart}, M. and {Mu{\~n}oz}, J.~A. and {Jim{\'e}nez-Vicente}, J.
	},
    title = "{Size of the Accretion Disk in the Graviationally Lensed Quasar SDSS J1004+4112 from the Statistics of Microlensing Magnifications}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1608.03831},
 keywords = {gravitational lensing: micro, gravitational lensing: strong, quasars: individual: SDSS J1004+4112},
     year = 2016,
    month = oct,
   volume = 830,
      eid = {149},
    pages = {149},
      doi = {10.3847/0004-637X/830/2/149},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...830..149F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Peterson2011,
   author = {{Peterson}, B.~M.},
    title = "{Masses of Black Holes in Active Galactic Nuclei: Implications for NLS1s}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1109.4181},
 primaryClass = "astro-ph.CO",
 keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
     year = 2011,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2011arXiv1109.4181P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shen2012,
   author = {{Shen}, Y. and {Kelly}, B.~C.},
    title = "{The Demographics of Broad-line Quasars in the Mass-Luminosity Plane. I. Testing FWHM-based Virial Black Hole Masses}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1107.4372},
 keywords = {black hole physics, galaxies: active, quasars: general, surveys},
     year = 2012,
    month = feb,
   volume = 746,
      eid = {169},
    pages = {169},
      doi = {10.1088/0004-637X/746/2/169},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...746..169S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Coatman2016,
   author = {{Coatman}, L. and {Hewett}, P.~C. and {Banerji}, M. and {Richards}, G.~T.
	},
    title = "{C IV emission-line properties and systematic trends in quasar black hole mass estimates}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1606.02726},
 keywords = {galaxies: evolution},
     year = 2016,
    month = sep,
   volume = 461,
    pages = {647-665},
      doi = {10.1093/mnras/stw1360},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.461..647C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marziani2012,
   author = {{Marziani}, P. and {Sulentic}, J.~W.},
    title = "{Estimating black hole masses in quasars using broad optical and UV emission lines}",
  journal = {\nar},
archivePrefix = "arXiv",
   eprint = {1108.5102},
     year = 2012,
    month = feb,
   volume = 56,
    pages = {49-63},
      doi = {10.1016/j.newar.2011.09.001},
   adsurl = {http://adsabs.harvard.edu/abs/2012NewAR..56...49M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kova2017,
   author = {{Kova{\v c}evi{\'c}-Doj{\v c}inovi{\'c}}, J. and {Mar{\v c}eta-Mandi{\'c}}, S. and 
	{Popovi{\'c}}, L.~{\v C}.},
    title = "{Black Hole Mass Estimation in the Type 1 AGN: H beta vs. Mg II lines and the role of Balmer continuum}",
  journal = {Frontiers in Astronomy and Space Sciences},
archivePrefix = "arXiv",
   eprint = {1707.08251},
 keywords = {galaxies: active, galaxies: nuclei, Quasars: supermassive black holes, techniques: spectroscopic, quasars: emission lines, Line: profiles},
     year = 2017,
    month = jul,
   volume = 4,
      eid = {7},
    pages = {7},
      doi = {10.3389/fspas.2017.00007},
   adsurl = {http://adsabs.harvard.edu/abs/2017FrASS...4....7K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Vestergaard2011,
   author = {{Vestergaard}, M. and {Denney}, K. and {Fan}, X. and {Jensen}, J.~J. and 
	{Kelly}, B.~C. and {Osmer}, P.~S. and {Peterson}, B.~M. and 
	{Tremonti}, C.~A.},
    title = "{Black hole mass estimations: limitations and uncertainties}",
booktitle = {Narrow-Line Seyfert 1 Galaxies and their Place in the Universe},
     year = 2011,
      eid = {38},
    pages = {38},
   adsurl = {http://adsabs.harvard.edu/abs/2011nlsg.confE..38V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kova2015,
   author = {{Kova{\v c}evi{\'c}-Doj{\v c}inovi{\'c}}, J. and {Popovi{\'c}}, L.~{\v C}.
	},
    title = "{The Connections Between the UV and Optical Fe ii Emission Lines in Type 1 AGNs}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1509.03679},
 keywords = {galaxies: active, quasars: emission lines},
     year = 2015,
    month = dec,
   volume = 221,
      eid = {35},
    pages = {35},
      doi = {10.1088/0067-0049/221/2/35},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJS..221...35K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Sulentic2000,
   author = {{Sulentic}, J.~W. and {Marziani}, P. and {Dultzin-Hacyan}, D.
	},
    title = "{Phenomenology of Broad Emission Lines in Active Galactic Nuclei}",
  journal = {\araa},
 keywords = {SEYFERT GALAXIES, QUASARS, ACCRETION DISKS, SPECTROSCOPY, EMISSION LINES, LINE FORMATION},
     year = 2000,
   volume = 38,
    pages = {521-571},
      doi = {10.1146/annurev.astro.38.1.521},
   adsurl = {http://adsabs.harvard.edu/abs/2000ARA%26A..38..521S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Motta2012,
   author = {{Motta}, V. and {Mediavilla}, E. and {Falco}, E. and {Mu{\~n}oz}, J.~A.
	},
    title = "{Measuring Microlensing Using Spectra of Multiply Lensed Quasars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1206.1582},
 keywords = {accretion, accretion disks, gravitational lensing: micro, gravitational lensing: strong, quasars: individual: HS0818+1227 Q0957+561 SDSS1004+4112 SDSS1029+2623 HE1104-1805},
     year = 2012,
    month = aug,
   volume = 755,
      eid = {82},
    pages = {82},
      doi = {10.1088/0004-637X/755/1/82},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...755...82M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sluse2012,
   author = {{Sluse}, D. and {Hutsem{\'e}kers}, D. and {Courbin}, F. and 
	{Meylan}, G. and {Wambsganss}, J.},
    title = "{Microlensing of the broad line region in 17 lensed quasars}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1206.0731},
 primaryClass = "astro-ph.CO",
 keywords = {gravitational lensing: micro, gravitational lensing: strong, line: formation, quasars: general, quasars: emission lines},
     year = 2012,
    month = aug,
   volume = 544,
      eid = {A62},
    pages = {A62},
      doi = {10.1051/0004-6361/201219125},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...544A..62S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wisotzki2003,
   author = {{Wisotzki}, L. and {Becker}, T. and {Christensen}, L. and {Helms}, A. and 
	{Jahnke}, K. and {Kelz}, A. and {Roth}, M.~M. and {Sanchez}, S.~F.
	},
    title = "{Integral-field spectrophotometry of the quadruple QSO HE 0435-1223: Evidence for microlensing}",
  journal = {\aap},
   eprint = {astro-ph/0307147},
 keywords = {quasars: individual: HE 0435-1223, quasars: general, gravitational lensing},
     year = 2003,
    month = sep,
   volume = 408,
    pages = {455-463},
      doi = {10.1051/0004-6361:20031004},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...408..455W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Inada2006,
   author = {{Inada}, N. and {Oguri}, M. and {Becker}, R.~H. and {White}, R.~L. and 
	{Gregg}, M.~D. and {Schechter}, P.~L. and {Kawano}, Y. and {Kochanek}, C.~S. and 
	{Richards}, G.~T. and {Schneider}, D.~P. and {Barentine}, J.~C. and 
	{Brewington}, H.~J. and {Brinkmann}, J. and {Harvanek}, M. and 
	{Kleinman}, S.~J. and {Krzesinski}, J. and {Long}, D. and {Neilsen}, Jr., E.~H. and 
	{Nitta}, A. and {Snedden}, S.~A. and {York}, D.~G.},
    title = "{SDSS J0806+2006 and SDSS J1353+1138: Two New Gravitationally Lensed Quasars from the Sloan Digital Sky Survey}",
  journal = {\aj},
   eprint = {astro-ph/0512239},
 keywords = {Gravitational Lensing, quasars: individual (SDSS J080623.70+200631.9), quasars: individual (SDSS J135306.35+113804.8)},
     year = 2006,
    month = apr,
   volume = 131,
    pages = {1934-1941},
      doi = {10.1086/500591},
   adsurl = {http://adsabs.harvard.edu/abs/2006AJ....131.1934I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schechter1998,
   author = {{Schechter}, P.~L. and {Gregg}, M.~D. and {Becker}, R.~H. and 
	{Helfand}, D.~J. and {White}, R.~L.},
    title = "{The First FIRST Gravitationally Lensed Quasar: FBQ 0951+2635}",
  journal = {\aj},
   eprint = {astro-ph/9710120},
 keywords = {GRAVITATIONAL LENSING, QUASARS: EMISSION LINE, QUASARS: INDIVIDUAL: FBQ0951+2635},
     year = 1998,
    month = apr,
   volume = 115,
    pages = {1371-1376},
      doi = {10.1086/300294},
   adsurl = {http://adsabs.harvard.edu/abs/1998AJ....115.1371S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Goicoechea2005,
   author = {{Goicoechea}, L.~J. and {Gil-Merino}, R. and {Ull{\'a}n}, A.
	},
    title = "{The dark halo of the main lens galaxy in QSO 0957 + 561}",
  journal = {\mnras},
   eprint = {astro-ph/0503610},
 keywords = {gravitational lensing, dust, extinction, galaxies: elliptical and lenticular, cD, galaxies: haloes, quasars: individual: QSO 0957 + 561, dark matter},
     year = 2005,
    month = jun,
   volume = 360,
    pages = {L60-L63},
      doi = {10.1111/j.1745-3933.2005.00046.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.360L..60G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Richards2004,
   author = {{Richards}, G.~T. and {Keeton}, C.~R. and {Pindor}, B. and {Hennawi}, J.~F. and 
	{Hall}, P.~B. and {Turner}, E.~L. and {Inada}, N. and {Oguri}, M. and 
	{Ichikawa}, S.-I. and {Becker}, R.~H. and {Gregg}, M.~D. and 
	{White}, R.~L. and {Wyithe}, J.~S.~B. and {Schneider}, D.~P. and 
	{Johnston}, D.~E. and {Frieman}, J.~A. and {Brinkmann}, J.},
    title = "{Microlensing of the Broad Emission Line Region in the Quadruple Lens SDSS J1004+4112}",
  journal = {\apj},
   eprint = {astro-ph/0402345},
 keywords = {Cosmology: Gravitational Lensing, Galaxies: Quasars: Emission Lines, Galaxies: Quasars: General, Galaxies: Quasars: Individual: Alphanumeric: SDSS J100434.91+411242.8},
     year = 2004,
    month = aug,
   volume = 610,
    pages = {679-685},
      doi = {10.1086/421868},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...610..679R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gomez2006,
   author = {{G{\'o}mez-{\'A}lvarez}, P. and {Mediavilla}, E. and {Mu{\~n}oz}, J.~A. and 
	{Arribas}, S. and {S{\'a}nchez}, S.~F. and {Oscoz}, A. and {Prada}, F. and 
	{Serra-Ricart}, M.},
    title = "{Recurrence of the Blue Wing Enhancements in the High-Ionization Lines of SDSS 1004+4112A}",
  journal = {\apjl},
   eprint = {astro-ph/0605522},
 keywords = {Cosmology: Gravitational Lensing, Galaxies: Quasars: Emission Lines, quasars: individual (SDSS 1004+4112)},
     year = 2006,
    month = jul,
   volume = 645,
    pages = {L5-L8},
      doi = {10.1086/506147},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...645L...5G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shalyapin2014,
   author = {{Shalyapin}, V.~N. and {Goicoechea}, L.~J.},
    title = "{Deep optical imaging and spectroscopy of the lens system SDSS J1339+1310}",
  journal = {\aap},
 keywords = {gravitational lensing: strong, gravitational lensing: micro, galaxies: halos, quasars: general, quasars: individual: SDSS J1339+1310},
     year = 2014,
    month = aug,
   volume = 568,
      eid = {A116},
    pages = {A116},
      doi = {10.1051/0004-6361/201323360},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...568A.116S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Morgan2004,
   author = {{Morgan}, N.~D. and {Caldwell}, J.~A.~R. and {Schechter}, P.~L. and 
	{Dressler}, A. and {Egami}, E. and {Rix}, H.-W.},
    title = "{WFI J2026-4536 and WFI J2033-4723: Two New Quadruple Gravitational Lenses}",
  journal = {\aj},
   eprint = {astro-ph/0312478},
 keywords = {Cosmology: Gravitational Lensing},
     year = 2004,
    month = may,
   volume = 127,
    pages = {2617-2630},
      doi = {10.1086/383295},
   adsurl = {http://adsabs.harvard.edu/abs/2004AJ....127.2617M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rojas2014,
   author = {{Rojas}, K. and {Motta}, V. and {Mediavilla}, E. and {Falco}, E. and 
	{Jim{\'e}nez-Vicente}, J. and {Mu{\~n}oz}, J.~A.},
    title = "{Strong Chromatic Microlensing in HE0047-1756 and SDSS1155+6346}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1409.8246},
 keywords = {gravitational lensing: micro, gravitational lensing: strong, quasars: individual: HE0047{\ndash}1756 SDSS1155+6346},
     year = 2014,
    month = dec,
   volume = 797,
      eid = {61},
    pages = {61},
      doi = {10.1088/0004-637X/797/1/61},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...797...61R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mediavilla2005,
   author = {{Mediavilla}, E. and {Mu{\~n}oz}, J.~A. and {Kochanek}, C.~S. and 
	{Falco}, E.~E. and {Arribas}, S. and {Motta}, V.},
    title = "{The First Precise Determination of an Optical-Far-Ultraviolet Extinction Curve Beyond the Local Group (z=0.83)}",
  journal = {\apj},
 keywords = {ISM: Dust, Extinction, Cosmology: Gravitational Lensing, Galaxies: Quasars: Individual: Alphanumeric: SBS 0909+532},
     year = 2005,
    month = feb,
   volume = 619,
    pages = {749-754},
      doi = {10.1086/426579},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...619..749M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eigenbrod2006,
   author = {{Eigenbrod}, A. and {Courbin}, F. and {Dye}, S. and {Meylan}, G. and 
	{Sluse}, D. and {Vuissoz}, C. and {Magain}, P.},
    title = "{COSMOGRAIL: the COSmological MOnitoring of GRAvItational Lenses.  II. SDSS J0924+0219: the redshift of the lensing galaxy,  the quasar spectral variability and the Einstein rings}",
  journal = {\aap},
   eprint = {astro-ph/0510641},
 keywords = {gravitational lensing, cosmology: cosmological parameters, quasars: individual: SDSSJ0924+0219, dark matter},
     year = 2006,
    month = jun,
   volume = 451,
    pages = {747-757},
      doi = {10.1051/0004-6361:20054423},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...451..747E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Oguri2005,
   author = {{Oguri}, M. and {Inada}, N. and {Hennawi}, J.~F. and {Richards}, G.~T. and 
	{Johnston}, D.~E. and {Frieman}, J.~A. and {Pindor}, B. and 
	{Strauss}, M.~A. and {Brunner}, R.~J. and {Becker}, R.~H. and 
	{Castander}, F.~J. and {Gregg}, M.~D. and {Hall}, P.~B. and 
	{Rix}, H.-W. and {Schneider}, D.~P. and {Bahcall}, N.~A. and 
	{Brinkmann}, J. and {York}, D.~G.},
    title = "{Discovery of Two Gravitationally Lensed Quasars with Image Separations of 3'' from the Sloan Digital Sky Survey}",
  journal = {\apj},
   eprint = {astro-ph/0411250},
 keywords = {Cosmology: Observations, Cosmology: Theory, Cosmology: Gravitational Lensing, Galaxies: Quasars: Individual: Alphanumeric: SDSS J100128.61+502756.9, Galaxies: Quasars: Individual: Alphanumeric: SDSS J120629.65+433217.6},
     year = 2005,
    month = mar,
   volume = 622,
    pages = {106-115},
      doi = {10.1086/428087},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...622..106O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Surdej1997,
   author = {{Surdej}, J. and {Claeskens}, J.-F. and {Remy}, M. and {Refsdal}, S. and 
	{Pirenne}, B. and {Prieto}, A. and {Vanderriest}, C.},
    title = "{HST confirmation of the lensed quasar J03.13.}",
  journal = {\aap},
 keywords = {, GRAVITATIONAL LENSING, QUASARS: INDIVIDUAL: J03.13 , TECHNIQUES: IMAGE PROCESSING},
     year = 1997,
    month = nov,
   volume = 327,
    pages = {L1-L4},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...327L...1S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chavushyan1997,
   author = {{Chavushyan}, V.~H. and {Vlasyuk}, V.~V. and {Stepanian}, J.~A. and 
	{Erastova}, L.~K.},
    title = "{SBS 1520+530: a new gravitationally lensed system at z=1.855.}",
  journal = {\aap},
 keywords = {GRAVITATIONAL LENSING, QUASARS: EMISSION-LINES, QUASARS: ABSOPRTION-LINES, QUASARS: INDIVIDUAL: SBS 1520+530},
     year = 1997,
    month = feb,
   volume = 318,
    pages = {L67-L70},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...318L..67C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wucknitz2003,
   author = {{Wucknitz}, O. and {Wisotzki}, L. and {Lopez}, S. and {Gregg}, M.~D.
	},
    title = "{Disentangling microlensing and differential extinction  in the double QSO <ASTROBJ>HE 0512-3329</ASTROBJ>}",
  journal = {\aap},
   eprint = {astro-ph/0304435},
 keywords = {gravitational lensing, dust, extinction, galaxies: ISM, quasars: individual: <ASTROBJ>HE 0512-3329</ASTROBJ>},
     year = 2003,
    month = jul,
   volume = 405,
    pages = {445-454},
      doi = {10.1051/0004-6361:20030608},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...405..445W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Motta2017,
	author = {{Motta}, V. and {Mediavilla}, E. and {Rojas}, K. and {Falco}, E.~E. and 
	{Jim{\'e}nez-Vicente}, J. and {Mu{\~n}oz}, J.~A.},
	title = "{Probing the Broad-Line Region and the Accretion Disk in the Lensed Quasars HE 0435-1223, WFI 2033-4723, and HE 2149-2745 Using Gravitational Microlensing}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1703.00400},
	keywords = {gravitational lensing: strong, quasars: emission lines, quasars: individual: HE 0435-1223, WFI 2033-4723, HE 2149-2745},
	year = 2017,
	month = feb,
	volume = 835,
	eid = {132},
	pages = {132},
	doi = {10.3847/1538-4357/835/2/132},
	adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...835..132M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eigenbrod2007,
	author = {{Eigenbrod}, A. and {Courbin}, F. and {Meylan}, G.},
	title = "{COSMOGRAIL: the COSmological MOnitoring of GRAvItational Lenses. VI. Redshift of the lensing galaxy in seven gravitationally lensed quasars}",
	journal = {\aap},
	eprint = {astro-ph/0612419},
	keywords = {gravitational lensing, cosmology: cosmological parameters},
	year = 2007,
	month = apr,
	volume = 465,
	pages = {51-56},
	doi = {10.1051/0004-6361:20066939},
	adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...465...51E},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Goicoechea2016,
	author = {{Goicoechea}, L.~J. and {Shalyapin}, V.~N.},
	title = "{Gravitational lens system SDSS J1339+1310: microlensing factory and time delay}",
	journal = {\aap},
	archivePrefix = "arXiv",
	eprint = {1609.07440},
	keywords = {gravitational lensing: strong, gravitational lensing: micro, quasars: individual: SDSS J1339+1310, cosmological parameters},
	year = 2016,
	month = dec,
	volume = 596,
	eid = {A77},
	pages = {A77},
	doi = {10.1051/0004-6361/201628790},
	adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...596A..77G},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burud2002,
	author = {{Burud}, I. and {Courbin}, F. and {Magain}, P. and {Lidman}, C. and 
	{Hutsem{\'e}kers}, D. and {Kneib}, J.-P. and {Hjorth}, J. and 
	{Brewer}, J. and {Pompei}, E. and {Germany}, L. and {Pritchard}, J. and 
	{Jaunsen}, A.~O. and {Letawe}, G. and {Meylan}, G.},
	title = "{An optical time-delay for the lensed BAL quasar HE 2149-2745}",
	journal = {\aap},
	eprint = {astro-ph/0112225},
	keywords = {GRAVITATIONAL LENSING, QUASARS: INDIVIDUAL: HE 2149-2745, COSMOLOGICAL PARAMETERS},
	year = 2002,
	month = jan,
	volume = 383,
	pages = {71-81},
	doi = {10.1051/0004-6361:20011731},
	adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...383...71B},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wisotzki1993,
	author = {{Wisotzki}, L. and {Koehler}, T. and {Kayser}, R. and {Reimers}, D.
	},
	title = "{The new double QSO HE 1104-1805: Gravitational lens with microlensing or binary quasar?}",
	journal = {\aap},
	keywords = {Absorption Spectra, Emission Spectra, Gravitational Lenses, Quasars, Disk Galaxies, Lyman Alpha Radiation, Red Shift, Stellar Magnitude, Stellar Spectrophotometry},
	year = 1993,
	month = oct,
	volume = 278,
	pages = {L15-L18},
	adsurl = {http://adsabs.harvard.edu/abs/1993A%26A...278L..15W},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wisotzki1995,
	author = {{Wisotzki}, L. and {Koehler}, T. and {Ikonomou}, M. and {Reimers}, D.
	},
	title = "{Spectral variability in the double QSO HE 1104-1805: further evidence for gravitational lensing.}",
	journal = {\aap},
	keywords = {QUASARS: GENERAL, QUASARS: EMISSION LINES, QUASARS: INDIDUAL: HE 1104-1805, GRAVITATIONAL LENSING},
	year = 1995,
	month = may,
	volume = 297,
	pages = {L59},
	adsurl = {http://adsabs.harvard.edu/abs/1995A%26A...297L..59W},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Abolmaso2012,
	author = {{Abolmasov}, P. and {Shakura}, N.~I.},
	title = "{Resolving the inner structure of QSO discs through fold-caustic-crossing events}",
	journal = {\mnras},
	archivePrefix = "arXiv",
	eprint = {1203.2656},
	primaryClass = "astro-ph.HE",
	keywords = {accretion, accretion discs, gravitational lensing: micro, quasars: individual: QSO J2237+0305, quasars: individual: SBS J1520+530},
	year = 2012,
	month = jun,
	volume = 423,
	pages = {676-693},
	doi = {10.1111/j.1365-2966.2012.20904.x},
	adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.423..676A},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Alcalde2002,
	author = {{Alcalde}, D. and {Mediavilla}, E. and {Moreau}, O. and {Mu{\~n}oz}, J.~A. and 
	{Libbrecht}, C. and {Goicoechea}, L.~J. and {Surdej}, J. and 
	{Puga}, E. and {De Rop}, Y. and {Barrena}, R. and {Gil-Merino}, R. and 
	{McLeod}, B.~A. and {Motta}, V. and {Oscoz}, A. and {Serra-Ricart}, M.
	},
	title = "{QSO 2237+0305 VR Light Curves from Gravitational LensES International Time Project Optical Monitoring}",
	journal = {\apj},
	eprint = {astro-ph/0204426},
	keywords = {Galaxies: Photometry, Cosmology: Gravitational Lensing, Galaxies: Quasars: Individual: Alphanumeric: Q2237+0305},
	year = 2002,
	month = jun,
	volume = 572,
	pages = {729-734},
	doi = {10.1086/340343},
	adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...572..729A},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Anguita2008,
	author = {{Anguita}, T. and {Schmidt}, R.~W. and {Turner}, E.~L. and {Wambsganss}, J. and 
	{Webster}, R.~L. and {Loomis}, K.~A. and {Long}, D. and {McMillan}, R.
	},
	title = "{The multiple quasar Q2237+0305 under a microlensing caustic}",
	journal = {\aap},
	archivePrefix = "arXiv",
	eprint = {0711.4265},
	keywords = {gravitational lensing, galaxies: quasars: individual: Q2237+0305, cosmology: observations, accretion, accretion disks},
	year = 2008,
	month = mar,
	volume = 480,
	pages = {327-334},
	doi = {10.1051/0004-6361:20078221},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...480..327A},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Assef2011,
	author = {{Assef}, R.~J. and {Denney}, K.~D. and {Kochanek}, C.~S. and 
	{Peterson}, B.~M. and {Koz{\l}owski}, S. and {Ageorges}, N. and 
	{Barrows}, R.~S. and {Buschkamp}, P. and {Dietrich}, M. and 
	{Falco}, E. and {Feiz}, C. and {Gemperlein}, H. and {Germeroth}, A. and 
	{Grier}, C.~J. and {Hofmann}, R. and {Juette}, M. and {Khan}, R. and 
	{Kilic}, M. and {Knierim}, V. and {Laun}, W. and {Lederer}, R. and 
	{Lehmitz}, M. and {Lenzen}, R. and {Mall}, U. and {Madsen}, K.~K. and 
	{Mandel}, H. and {Martini}, P. and {Mathur}, S. and {Mogren}, K. and 
	{Mueller}, P. and {Naranjo}, V. and {Pasquali}, A. and {Polsterer}, K. and 
	{Pogge}, R.~W. and {Quirrenbach}, A. and {Seifert}, W. and {Stern}, D. and 
	{Shappee}, B. and {Storz}, C. and {Van Saders}, J. and {Weiser}, P. and 
	{Zhang}, D.},
	title = "{Black Hole Mass Estimates Based on C IV are Consistent with Those Based on the Balmer Lines}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1009.1145},
	keywords = {galaxies: active, gravitational lensing: strong, quasars: emission lines},
	year = 2011,
	month = dec,
	volume = 742,
	eid = {93},
	pages = {93},
	doi = {10.1088/0004-637X/742/2/93},
	adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...742...93A},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chang1979,
	author = {{Chang}, K. and {Refsdal}, S.},
	title = "{Flux variations of QSO 0957+561 A, B and image splitting by stars near the light path}",
	journal = {\nat},
	keywords = {Binary Stars, Gravitational Lenses, Optical Paths, Quasars, Radiant Flux Density, Point Sources, Star Distribution},
	year = 1979,
	month = dec,
	volume = 282,
	pages = {561-564},
	doi = {10.1038/282561a0},
	adsurl = {http://adsabs.harvard.edu/abs/1979Natur.282..561C},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chang1984,
	author = {{Chang}, K. and {Refsdal}, S.},
	title = "{Star disturbances in gravitational lens galaxies}",
	journal = {\aap},
	keywords = {Cosmology, Galaxies, Gravitational Lenses, Light Curve, Stellar Gravitation, Gravitational Effects, Quasars},
	year = 1984,
	month = mar,
	volume = 132,
	pages = {168-178},
	adsurl = {http://adsabs.harvard.edu/abs/1984A%26A...132..168C},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eigenbrod2008a,
	author = {{Eigenbrod}, A. and {Courbin}, F. and {Sluse}, D. and {Meylan}, G. and 
	{Agol}, E.},
	title = "{Microlensing variability in the gravitationally lensed quasar QSO 2237+0305 {\equiv} the Einstein Cross . I. Spectrophotometric monitoring with the VLT}",
	journal = {\aap},
	archivePrefix = "arXiv",
	eprint = {0709.2828},
	keywords = {gravitational lensing, galaxies: quasars: general, galaxies: quasars: emission, line, quasars: individual: QSO 2237+0305, Einstein Cross},
	year = 2008,
	month = mar,
	volume = 480,
	pages = {647-661},
	doi = {10.1051/0004-6361:20078703},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...480..647E},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eigenbrod2008b,
	author = {{Eigenbrod}, A. and {Courbin}, F. and {Meylan}, G. and {Agol}, E. and 
	{Anguita}, T. and {Schmidt}, R.~W. and {Wambsganss}, J.},
	title = "{Microlensing variability in the gravitationally lensed quasar QSO 2237+0305 {\equiv} the Einstein Cross. II. Energy profile of the accretion disk}",
	journal = {\aap},
	archivePrefix = "arXiv",
	eprint = {0810.0011},
	keywords = {gravitational lensing, quasars: individual: QSO 2237+0305, accretion, accretion disks},
	year = 2008,
	month = nov,
	volume = 490,
	pages = {933-943},
	doi = {10.1051/0004-6361:200810729},
	adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...490..933E},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gil-Merino2005,
	author = {{Gil-Merino}, R. and {Wambsganss}, J. and {Goicoechea}, L.~J. and 
	{Lewis}, G.~F.},
	title = "{Limits on the transverse velocity of the lensing galaxy in Q2237+0305 from the lack of strong microlensing variability}",
	journal = {\aap},
	eprint = {astro-ph/0411239},
	keywords = {gravitational lensing, galaxies: quasars: individual: Q2237+0305, methods: numerical},
	year = 2005,
	month = mar,
	volume = 432,
	pages = {83-89},
	doi = {10.1051/0004-6361:20047123},
	adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...432...83G},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gil-Merino2006,
	author = {{Gil-Merino}, R. and {Gonz{\'a}lez-Cadelo}, J. and {Goicoechea}, L.~J. and 
	{Shalyapin}, V.~N. and {Lewis}, G.~F.},
	title = "{Is there a caustic crossing in the lensed quasar Q2237+0305 observational data record?}",
	journal = {\mnras},
	eprint = {astro-ph/0607162},
	keywords = {gravitational lensing: quasars: individual: Q2237+0305, gravitational lensing, quasars: individual: Q2237+0305},
	year = 2006,
	month = sep,
	volume = 371,
	pages = {1478-1482},
	doi = {10.1111/j.1365-2966.2006.10782.x},
	adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.371.1478G},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Goicoechea2003,
	author = {{Goicoechea}, L.~J. and {Alcalde}, D. and {Mediavilla}, E. and 
	{Mu{\~n}oz}, J.~A.},
	title = "{Determination of the properties of the central engine in microlensed QSOs}",
	journal = {\aap},
	eprint = {astro-ph/0210291},
	keywords = {gravitational lensing, galaxies: nuclei, quasars: general, quasars: individual: Q2237+0305},
	year = 2003,
	month = jan,
	volume = 397,
	pages = {517-525},
	doi = {10.1051/0004-6361:20021535},
	adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...397..517G},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kochanek2004,
	author = {{Kochanek}, C.~S.},
	title = "{Quantitative Interpretation of Quasar Microlensing Light Curves}",
	journal = {\apj},
	eprint = {astro-ph/0307422},
	keywords = {Accretion, Accretion Disks, Cosmology: Dark Matter, Cosmology: Gravitational Lensing, Galaxies: Quasars: Individual: Alphanumeric: Q2237+0305, Stars: Luminosity Function, Mass Function},
	year = 2004,
	month = apr,
	volume = 605,
	pages = {58-77},
	doi = {10.1086/382180},
	adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...605...58K},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Koptelova2007,
	author = {{Koptelova}, E. and {Shimanovskaya}, E. and {Artamonov}, B. and 
	{Yagola}, A.},
	title = "{Analysis of the Q2237+0305 light-curve variability with regularization technique}",
	journal = {\mnras},
	keywords = {gravitational lensing, quasars: individual: Q2237+0305},
	year = 2007,
	month = nov,
	volume = 381,
	pages = {1655-1662},
	doi = {10.1111/j.1365-2966.2007.12335.x},
	adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.381.1655K},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Marshall2010,
	author = {{Marshall}, P.~J. and {Bradac}, M. and {Chartas}, G. and {Dobler}, G. and 
	{Eliasdottir}, A. and {Falco}, E. and {Fassnacht}, C.~D. and 
	{Jee}, M.~J. and {Keeton}, C.~R. and {Oguri}, M. and {Tyson}, J.~A. and 
	{LSST Strong Lensing Science Collaboration}},
	title = "{Strong Gravitational Lensing with LSST}",
	booktitle = {American Astronomical Society Meeting Abstracts \#215},
	year = 2010,
	series = {Bulletin of the American Astronomical Society},
	volume = 42,
	month = jan,
	eid = {401.15},
	pages = {219},
	adsurl = {http://adsabs.harvard.edu/abs/2010AAS...21540115M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mediavilla2006,
	author = {{Mediavilla}, E. and {Mu{\~n}oz}, J.~A. and {Lopez}, P. and 
	{Mediavilla}, T. and {Abajas}, C. and {Gonzalez-Morcillo}, C. and 
	{Gil-Merino}, R.},
	title = "{A Fast and Very Accurate Approach to the Computation of Microlensing Magnification Patterns Based on Inverse Polygon Mapping}",
	journal = {\apj},
	keywords = {Cosmology: Gravitational Lensing},
	year = 2006,
	month = dec,
	volume = 653,
	pages = {942-953},
	doi = {10.1086/508796},
	adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...653..942M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Mediavilla2011,
	author = {{Mediavilla}, E. and {Mediavilla}, T. and {Mu{\~n}oz}, J.~A. and 
	{Ariza}, O. and {Lopez}, P. and {Gonzalez-Morcillo}, C. and 
	{Jimenez-Vicente}, J.},
	title = "{New Developments on Inverse Polygon Mapping to Calculate Gravitational Lensing Magnification Maps: Optimized Computations}",
	journal = {\apj},
	keywords = {gravitational lensing: micro},
	year = 2011,
	month = nov,
	volume = 741,
	eid = {42},
	pages = {42},
	doi = {10.1088/0004-637X/741/1/42},
	adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...741...42M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mediavilla2015,
	author = {{Mediavilla}, E. and {Jimenez-Vicente}, J. and {Mu{\~n}oz}, J.~A. and 
	{Mediavilla}, T. and {Ariza}, O.},
	title = "{Statistics of Microlensing Caustic Crossings in Q 2237+0305: Peculiar Velocity of the Lens Galaxy and Accretion Disk Size}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1411.2745},
	keywords = {gravitational lensing: micro, quasars: general},
	year = 2015,
	month = jan,
	volume = 798,
	eid = {138},
	pages = {138},
	doi = {10.1088/0004-637X/798/2/138},
	adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798..138M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mosquera2009,
	author = {{Mosquera}, A.~M. and {Mu{\~n}oz}, J.~A. and {Mediavilla}, E.
	},
	title = "{Detection of Chromatic Microlensing in Q 2237 + 0305 A}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {0810.1626},
	keywords = {accretion, accretion disks, gravitational lensing, quasars: individual: Q 2237 + 0305},
	year = 2009,
	month = feb,
	volume = 691,
	pages = {1292-1299},
	doi = {10.1088/0004-637X/691/2/1292},
	adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...691.1292M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mosquera2011,
	author = {{Mosquera}, A.~M. and {Kochanek}, C.~S.},
	title = "{The Microlensing Properties of a Sample of 87 Lensed Quasars}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1104.2356},
	primaryClass = "astro-ph.CO",
	keywords = {accretion, accretion disks, gravitational lensing: micro, quasars: general},
	year = 2011,
	month = sep,
	volume = 738,
	eid = {96},
	pages = {96},
	doi = {10.1088/0004-637X/738/1/96},
	adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...738...96M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Poindexter2010,
	author = {{Poindexter}, S. and {Kochanek}, C.~S.},
	title = "{Microlensing Evidence that a Type 1 Quasar is Viewed Face-On}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {0910.3669},
	keywords = {gravitational lensing: micro, methods: numerical, quasars: individual: Q2237+0305},
	year = 2010,
	month = mar,
	volume = 712,
	pages = {668-673},
	doi = {10.1088/0004-637X/712/1/668},
	adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...712..668P},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shakura1973,
	author = {{Shakura}, N.~I. and {Sunyaev}, R.~A.},
	title = "{Black holes in binary systems. Observational appearance.}",
	journal = {\aap},
	year = 1973,
	volume = 24,
	pages = {337-355},
	adsurl = {http://adsabs.harvard.edu/abs/1973A%26A....24..337S},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shalyapin2001,
	author = {{Shalyapin}, V.~N.},
	title = "{Caustic Crossing in the Gravitational Lens Q2237+0305}",
	journal = {Astronomy Letters},
	eprint = {astro-ph/0102384},
	keywords = {QUASARS, GRAVITATIONAL LENSES, ACCRETION DISKS},
	year = 2001,
	month = mar,
	volume = 27,
	pages = {150-155},
	doi = {10.1134/1.1351558},
	adsurl = {http://adsabs.harvard.edu/abs/2001AstL...27..150S},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shalyapin2002,
	author = {{Shalyapin}, V.~N. and {Goicoechea}, L.~J. and {Alcalde}, D. and 
	{Mediavilla}, E. and {Mu{\~n}oz}, J.~A. and {Gil-Merino}, R.
	},
	title = "{The Nature and Size of the Optical Continuum Source in QSO 2237+0305}",
	journal = {\apj},
	eprint = {astro-ph/0207236},
	keywords = {Accretion, Accretion Disks, Galaxies: Active, Cosmology: Gravitational Lensing, Galaxies: Quasars: Individual: Alphanumeric: Q2237+0305},
	year = 2002,
	month = nov,
	volume = 579,
	pages = {127-135},
	doi = {10.1086/342753},
	adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...579..127S},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schneider1987,
	author = {{Schneider}, P. and {Weiss}, A.},
	title = "{A gravitational lens origin for AGN-variability? Consequences of micro-lensing}",
	journal = {\aap},
	keywords = {Active Galactic Nuclei, Astronomical Models, Gravitational Lenses, Light Curve, Quasars, Star Distribution, Optical Thickness, Radiant Flux Density, Wave Amplification},
	year = 1987,
	month = jan,
	volume = 171,
	pages = {49-65},
	adsurl = {http://adsabs.harvard.edu/abs/1987A%26A...171...49S},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sluse2011,
	author = {{Sluse}, D. and {Schmidt}, R. and {Courbin}, F. and {Hutsem{\'e}kers}, D. and 
	{Meylan}, G. and {Eigenbrod}, A. and {Anguita}, T. and {Agol}, E. and 
	{Wambsganss}, J.},
	title = "{Zooming into the broad line region of the gravitationally lensed quasar QSO 2237 + 0305 {\equiv} the Einstein Cross. III. Determination of the size and structure of the C iv and C iii] emitting regions using microlensing}",
	journal = {\aap},
	archivePrefix = "arXiv",
	eprint = {1012.2871},
	keywords = {gravitational lensing: micro, gravitational lensing: strong, quasars: general, quasars: emission lines, quasars: individual: QSO 2237 + 0305, line: formation},
	year = 2011,
	month = apr,
	volume = 528,
	eid = {A100},
	pages = {A100},
	doi = {10.1051/0004-6361/201016110},
	adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...528A.100S},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Udalski2006,
	author = {{Udalski}, A. and {Szymanski}, M.~K. and {Kubiak}, M. and {Pietrzynski}, G. and 
	{Soszynski}, I. and {Zebrun}, K. and {Szewczyk}, O. and {Wyrzykowski}, L. and 
	{Ulaczyk}, K. and {Wi{\^e}ckowski}, T.},
	title = "{The Optical Gravitational Lensing Experiment. OGLE-III Long Term Monitoring of the Gravitational Lens QSO 2237+0305}",
	journal = {\actaa},
	eprint = {astro-ph/0701300},
	keywords = {Gravitational lensing, quasars: individual: QSO 2237+0305},
	year = 2006,
	month = dec,
	volume = 56,
	pages = {293-305},
	adsurl = {http://adsabs.harvard.edu/abs/2006AcA....56..293U},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Wambsganss2006,
	author = {{Wambsganss}, J.},
	title = "{Part 4: Gravitational microlensing}",
	keywords = {Gravitational Microlensing, Extrasolar Planets},
	booktitle = {Saas-Fee Advanced Course 33: Gravitational Lensing: Strong, Weak and Micro},
	year = 2006,
	editor = {{Meylan}, G. and {Jetzer}, P. and {North}, P. and {Schneider}, P. and 
	{Kochanek}, C.~S. and {Wambsganss}, J.},
	pages = {453-540},
	adsurl = {http://adsabs.harvard.edu/abs/2006glsw.conf..453W},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wozniak2000,
	author = {{Wo{\'z}niak}, P.~R. and {Alard}, C. and {Udalski}, A. and {Szyma{\'n}ski}, M. and 
	{Kubiak}, M. and {Pietrzy{\'n}ski}, G. and {Zebru{\'n}}, K.},
	title = "{The Optical Gravitational Lensing Experiment Monitoring of QSO 2237+0305}",
	journal = {\apj},
	eprint = {astro-ph/9904329},
	keywords = {GALAXIES: PHOTOMETRY, COSMOLOGY: GRAVITATIONAL LENSING, QUASARS: INDIVIDUAL (Q2237+0305), Galaxies: Photometry, Cosmology: Gravitational Lensing, quasars: individual (Q2237+0305)},
	year = 2000,
	month = jan,
	volume = 529,
	pages = {88-92},
	doi = {10.1086/308258},
	adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...529...88W},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wyithe1999,
	author = {{Wyithe}, J.~S.~B. and {Webster}, R.~L. and {Turner}, E.~L.},
	title = "{A measurement of the transverse velocity of Q2237+0305}",
	journal = {\mnras},
	eprint = {astro-ph/9901341},
	year = 1999,
	month = oct,
	volume = 309,
	pages = {261-272},
	doi = {10.1046/j.1365-8711.1999.02844.x},
	adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.309..261W},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wyithe2000,
	author = {{Wyithe}, J.~S.~B. and {Webster}, R.~L. and {Turner}, E.~L.},
	title = "{Interpretation of the OGLE Q2237+0305 microlensing light curve (1997-1999)}",
	journal = {\mnras},
	eprint = {astro-ph/0001307},
	keywords = {QUASARS: INDIVIDUAL: Q2237+0305, GRAVITATIONAL LENSING},
	year = 2000,
	month = nov,
	volume = 318,
	pages = {1120-1130},
	doi = {10.1046/j.1365-8711.2000.03747.x},
	adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.318.1120W},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Guerras2013,
  author={E. Guerras and E. Mediavilla and J. Jimenez-Vicente and C. S. Kochanek and J. A. Muñoz and E. Falco and V. Motta},
  title={Microlensing of Quasar Broad Emission Lines: Constraints on Broad Line Region Size},
  journal={The Astrophysical Journal},
  volume={764},
  number={2},
  pages={160},
  url={http://stacks.iop.org/0004-637X/764/i=2/a=160},
  year={2013},
  abstract={We measure the differential microlensing of the broad emission lines between 18 quasar image pairs in 16 gravitational lenses. We find that the broad emission lines are in general weakly microlensed. The results show, at a modest level of confidence (1.8σ), that high ionization lines such as C IV are more strongly microlensed than low ionization lines such as Hβ, indicating that the high ionization line emission regions are more compact. If we statistically model the distribution of microlensing magnifications, we obtain estimates for the broad line region size of r s = 24 +22 –15 and r s = 55 +150 –35 lt-day (90% confidence) for the high and low ionization lines, respectively. When the samples are divided into higher and lower luminosity quasars, we find that the line emission regions of more luminous quasars are larger, with a slope consistent with the expected scaling from photoionization models. Our estimates also agree well with the results from local reveberation mapping studies.}
}
	
@ARTICLE{Fine2010,
   author = {{Fine}, S. and {Croom}, S.~M. and {Bland-Hawthorn}, J. and {Pimbblet}, K.~A. and 
	{Ross}, N.~P. and {Schneider}, D.~P. and {Shanks}, T.},
    title = "{The CIV linewidth distribution for quasars and its implications for broad-line region dynamics and virial mass estimation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1005.5287},
 keywords = {galaxies: active, quasars: absorption lines, quasars: emission lines, quasars: general},
     year = 2010,
    month = dec,
   volume = 409,
    pages = {591-610},
      doi = {10.1111/j.1365-2966.2010.17107.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.409..591F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jim2015,
   author = {{Jim{\'e}nez-Vicente}, J. and {Mediavilla}, E. and {Kochanek}, C.~S. and 
	{Mu{\~n}oz}, J.~A.},
    title = "{Probing the Dark Matter Radial Profile in Lens Galaxies and the Size of X-Ray Emitting Region in Quasars with Microlensing}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1502.00394},
 keywords = {accretion, accretion disks, galaxies: stellar content, gravitational lensing: micro, quasars: general},
     year = 2015,
    month = jun,
   volume = 806,
      eid = {251},
    pages = {251},
      doi = {10.1088/0004-637X/806/2/251},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...806..251J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vestergaard2001,
   author = {{Vestergaard}, M. and {Wilkes}, B.~J.},
    title = "{An Empirical Ultraviolet Template for Iron Emission in Quasars as Derived from I Zwicky 1}",
  journal = {\apjs},
   eprint = {astro-ph/0104320},
 keywords = {Galaxies: Active, Galaxies: Individual: Alphanumeric: I Zw 1, Galaxies: Seyfert, Methods: Data Analysis, Galaxies: Quasars: Emission Lines},
     year = 2001,
    month = may,
   volume = 134,
    pages = {1-33},
      doi = {10.1086/320357},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJS..134....1V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{VandenBerk2001,
   author = {{Vanden Berk}, D.~E. and {Richards}, G.~T. and {Bauer}, A. and 
	{Strauss}, M.~A. and {Schneider}, D.~P. and {Heckman}, T.~M. and 
	{York}, D.~G. and {Hall}, P.~B. and {Fan}, X. and {Knapp}, G.~R. and 
	{Anderson}, S.~F. and {Annis}, J. and {Bahcall}, N.~A. and {Bernardi}, M. and 
	{Briggs}, J.~W. and {Brinkmann}, J. and {Brunner}, R. and {Burles}, S. and 
	{Carey}, L. and {Castander}, F.~J. and {Connolly}, A.~J. and 
	{Crocker}, J.~H. and {Csabai}, I. and {Doi}, M. and {Finkbeiner}, D. and 
	{Friedman}, S. and {Frieman}, J.~A. and {Fukugita}, M. and {Gunn}, J.~E. and 
	{Hennessy}, G.~S. and {Ivezi{\'c}}, {\v Z}. and {Kent}, S. and 
	{Kunszt}, P.~Z. and {Lamb}, D.~Q. and {Leger}, R.~F. and {Long}, D.~C. and 
	{Loveday}, J. and {Lupton}, R.~H. and {Meiksin}, A. and {Merelli}, A. and 
	{Munn}, J.~A. and {Newberg}, H.~J. and {Newcomb}, M. and {Nichol}, R.~C. and 
	{Owen}, R. and {Pier}, J.~R. and {Pope}, A. and {Rockosi}, C.~M. and 
	{Schlegel}, D.~J. and {Siegmund}, W.~A. and {Smee}, S. and {Snir}, Y. and 
	{Stoughton}, C. and {Stubbs}, C. and {SubbaRao}, M. and {Szalay}, A.~S. and 
	{Szokoly}, G.~P. and {Tremonti}, C. and {Uomoto}, A. and {Waddell}, P. and 
	{Yanny}, B. and {Zheng}, W.},
    title = "{Composite Quasar Spectra from the Sloan Digital Sky Survey}",
  journal = {\aj},
   eprint = {astro-ph/0105231},
 keywords = {Galaxies: Quasars: Emission Lines, Galaxies: Quasars: General},
     year = 2001,
    month = aug,
   volume = 122,
    pages = {549-564},
      doi = {10.1086/321167},
   adsurl = {http://adsabs.harvard.edu/abs/2001AJ....122..549V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wisotzki2004,
   author = {{Wisotzki}, L. and {Schechter}, P.~L. and {Chen}, H.-W. and 
	{Richstone}, D. and {Jahnke}, K. and {S{\'a}nchez}, S.~F. and 
	{Reimers}, D.},
    title = "{HE 0047-1756: A new gravitationally lensed double QSO}",
  journal = {\aap},
   eprint = {astro-ph/0403475},
 keywords = {quasars: individual: HE 0047-1756, quasars: general, gravitational lensing},
     year = 2004,
    month = may,
   volume = 419,
    pages = {L31-L34},
      doi = {10.1051/0004-6361:20040131},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...419L..31W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Abajas2002,
   author = {{Abajas}, C. and {Mediavilla}, E. and {Mu{\~n}oz}, J.~A. and 
	{Popovi{\'c}}, L.~{\v C}. and {Oscoz}, A.},
    title = "{The Influence of Gravitational Microlensing on the Broad Emission Lines of Quasars}",
  journal = {\apj},
   eprint = {astro-ph/0205407},
 keywords = {Cosmology: Gravitational Lensing, Galaxies: Quasars: Emission Lines},
     year = 2002,
    month = sep,
   volume = 576,
    pages = {640-652},
      doi = {10.1086/341793},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...576..640A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chang1979,
	author = {{Chang}, K. and {Refsdal}, S.},
	title = "{Flux variations of QSO 0957+561 A, B and image splitting by stars near the light path}",
	journal = {\nat},
	keywords = {Binary Stars, Gravitational Lenses, Optical Paths, Quasars, Radiant Flux Density, Point Sources, Star Distribution},
	year = 1979,
	month = dec,
	volume = 282,
	pages = {561-564},
	doi = {10.1038/282561a0},
	adsurl = {http://adsabs.harvard.edu/abs/1979Natur.282..561C},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pooley2007,
	author = {{Pooley}, D. and {Blackburne}, J.~A. and {Rappaport}, S. and 
	{Schechter}, P.~L.},
	title = "{X-Ray and Optical Flux Ratio Anomalies in Quadruply Lensed Quasars. I. Zooming in on Quasar Emission Regions}",
	journal = {\apj},
	eprint = {astro-ph/0607655},
	keywords = {Cosmology: Gravitational Lensing, Galaxies: Quasars: General},
	year = 2007,
	month = may,
	volume = 661,
	pages = {19-29},
	doi = {10.1086/512115},
	adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...661...19P},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Blackburne2011,
	author = {{Blackburne}, J.~A. and {Pooley}, D. and {Rappaport}, S. and 
	{Schechter}, P.~L.},
	title = "{Sizes and Temperature Profiles of Quasar Accretion Disks from Chromatic Microlensing}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1007.1665},
	primaryClass = "astro-ph.CO",
	keywords = {accretion, accretion disks, gravitational lensing: strong, quasars: general},
	year = 2011,
	month = mar,
	volume = 729,
	eid = {34},
	pages = {34},
	doi = {10.1088/0004-637X/729/1/34},
	adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...729...34B},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mosquera2011,
	author = {{Mosquera}, A.~M. and {Kochanek}, C.~S.},
	title = "{The Microlensing Properties of a Sample of 87 Lensed Quasars}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1104.2356},
	primaryClass = "astro-ph.CO",
	keywords = {accretion, accretion disks, gravitational lensing: micro, quasars: general},
	year = 2011,
	month = sep,
	volume = 738,
	eid = {96},
	pages = {96},
	doi = {10.1088/0004-637X/738/1/96},
	adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...738...96M},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Congdon2005,
   author = {{Congdon}, A.~B. and {Keeton}, C.~R.},
    title = "{Multipole models of four-image gravitational lenses with anomalous flux ratios}",
  journal = {\mnras},
   eprint = {astro-ph/0510232},
 keywords = {gravitational lensing, galaxies: haloes, galaxies: structure, dark matter},
     year = 2005,
    month = dec,
   volume = 364,
    pages = {1459-1466},
      doi = {10.1111/j.1365-2966.2005.09699.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.364.1459C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wambsganss1998,
   author = {{Wambsganss}, J.},
    title = "{Gravitational Lensing in Astronomy}",
  journal = {Living Reviews in Relativity},
   eprint = {astro-ph/9812021},
     year = 1998,
    month = nov,
   volume = 1,
      eid = {12},
    pages = {12},
      doi = {10.12942/lrr-1998-12},
   adsurl = {http://adsabs.harvard.edu/abs/1998LRR.....1...12W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{Schmidt2010,
author="Schmidt, R. W.
and Wambsganss, J.",
title="Quasar microlensing",
journal="General Relativity and Gravitation",
year="2010",
month="Sep",
day="01",
volume="42",
number="9",
pages="2127--2150",
issn="1572-9532",
doi="10.1007/s10714-010-0956-x",
url="https://doi.org/10.1007/s10714-010-0956-x"
}

@PHDTHESIS{Nemiroff1987,
   author = {{Nemiroff}, R.~J.},
    title = "{Prediction and analysis of basic gravitational microlensing phenomena}",
 keywords = {Active Galactic Nuclei, Astronomical Models, Formalism, Galactic Structure, Gravitational Lenses, Quasars, Emission Spectra, Light Curve, Stellar Gravitation},
   school = {Pennsylvania Univ., Philadelphia.},
     year = 1987,
    month = December,
      doi = {10.5281/zenodo.33974},
   adsurl = {http://adsabs.harvard.edu/abs/1987PhDT........12N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schneider1990,
   author = {{Schneider}, P. and {Wambsganss}, J.},
    title = "{Are the broad emission lines of quasars affected by gravitational microlensing?}",
  journal = {\aap},
 keywords = {Emission Spectra, Gravitational Lenses, Line Spectra, Quasars, Active Galactic Nuclei, Gravitational Effects, Stellar Radiation},
     year = 1990,
    month = oct,
   volume = 237,
    pages = {42-53},
   adsurl = {http://adsabs.harvard.edu/abs/1990A%26A...237...42S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lewis2004,
   author = {{Lewis}, G.~F. and {Ibata}, R.~A.},
    title = "{Gravitational microlensing of quasar broad-line regions at large optical depths}",
  journal = {\mnras},
   eprint = {astro-ph/0310818},
 keywords = {gravitational lensing, quasars: emission lines, quasars: individual: Q2237+0305},
     year = 2004,
    month = feb,
   volume = 348,
    pages = {24-33},
      doi = {10.1111/j.1365-2966.2004.07349.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.348...24L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Millon2020XIX,
       author = {{Millon}, M. and {Courbin}, F. and {Bonvin}, V. and {Paic}, E. and {Meylan}, G. and {Tewes}, M. and {Sluse}, D. and {Magain}, P. and {Chan}, J.~H.~H. and {Galan}, A. and {Joseph}, R. and {Lemon}, C. and {Tihhonova}, O. and {Anderson}, R.~I. and {Marmier}, M. and {Chazelas}, B. and {Lendl}, M. and {Triaud}, A.~H.~M.~J. and {Wyttenbach}, A.},
        title = "{COSMOGRAIL. XIX. Time delays in 18 strongly lensed quasars from 15 years of optical monitoring}",
      journal = {\aap},
     keywords = {gravitational lensing: strong, cosmology: observations, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = aug,
       volume = {640},
          eid = {A105},
        pages = {A105},
          doi = {10.1051/0004-6361/202037740},
archivePrefix = {arXiv},
       eprint = {2002.05736},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...640A.105M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Millon2020,
       author = {{Millon}, M. and {Courbin}, F. and {Bonvin}, V. and {Buckley-Geer}, E. and {Fassnacht}, C.~D. and {Frieman}, J. and {Marshall}, P.~J. and {Suyu}, S.~H. and {Treu}, T. and {Anguita}, T. and {Motta}, V. and {Agnello}, A. and {Chan}, J.~H.~H. and {Chao}, D.~C. -Y. and {Chijani}, M. and {Gilman}, D. and {Gilmore}, K. and {Lemon}, C. and {Lucey}, J.~R. and {Melo}, A. and {Paic}, E. and {Rojas}, K. and {Sluse}, D. and {Williams}, P.~R. and {Hempel}, A. and {Kim}, S. and {Lachaume}, R. and {Rabus}, M.},
        title = "{TDCOSMO. II. Six new time delays in lensed quasars from high-cadence monitoring at the MPIA 2.2 m telescope}",
      journal = {\aap},
     keywords = {gravitational lensing: strong, methods: data analysis, cosmological parameters, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = oct,
       volume = {642},
          eid = {A193},
        pages = {A193},
          doi = {10.1051/0004-6361/202038698},
archivePrefix = {arXiv},
       eprint = {2006.10066},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...642A.193M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hainline2013,
       author = {{Hainline}, Laura J. and {Morgan}, Christopher W. and {MacLeod}, Chelsea L. and {Landaal}, Zachary D. and {Kochanek}, C.~S. and {Harris}, Hugh C. and {Tilleman}, Trudy and {Goicoechea}, L.~J. and {Shalyapin}, V.~N. and {Falco}, Emilio E.},
        title = "{Time Delay and Accretion Disk Size Measurements in the Lensed Quasar SBS 0909+532 from Multiwavelength Microlensing Analysis}",
      journal = {\apj},
     keywords = {accretion, accretion disks, gravitational lensing: micro, gravitational lensing: strong, quasars: individual: SBS 0909+532, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = sep,
       volume = {774},
       number = {1},
          eid = {69},
        pages = {69},
          doi = {10.1088/0004-637X/774/1/69},
archivePrefix = {arXiv},
       eprint = {1307.3254},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...774...69H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fohlmeister2008,
       author = {{Fohlmeister}, J. and {Kochanek}, C.~S. and {Falco}, E.~E. and {Morgan}, C.~W. and {Wambsganss}, J.},
        title = "{The Rewards of Patience: An 822 Day Time Delay in the Gravitational Lens SDSS J1004+4112}",
      journal = {\apj},
     keywords = {cosmology: observations, gravitational lensing, quasars: individual: SDSS J1004+4112, Astrophysics},
         year = 2008,
        month = apr,
       volume = {676},
       number = {2},
        pages = {761-766},
          doi = {10.1086/528789},
archivePrefix = {arXiv},
       eprint = {0710.1634},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...676..761F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jakobsson2005,
       author = {{Jakobsson}, P. and {Hjorth}, J. and {Burud}, I. and {Letawe}, G. and {Lidman}, C. and {Courbin}, F.},
        title = "{An optical time delay for the double gravitational lens system FBQ 0951+2635}",
      journal = {\aap},
     keywords = {gravitational lensing, galaxies: quasars: individual: FBQ 0951+2635, cosmology: cosmological parameters, Astrophysics},
         year = 2005,
        month = feb,
       volume = {431},
        pages = {103-109},
          doi = {10.1051/0004-6361:20041432},
archivePrefix = {arXiv},
       eprint = {astro-ph/0409444},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...431..103J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shalyapin2008,
       author = {{Shalyapin}, V.~N. and {Goicoechea}, L.~J. and {Koptelova}, E. and {Ull{\'a}n}, A. and {Gil-Merino}, R.},
        title = "{New two-colour light curves of Q0957+561: time delays and the origin of intrinsic variations}",
      journal = {\aap},
     keywords = {techniques: photometric, gravitational lensing, black hole physics, quasars: individual:, Q0957+561, Astrophysics},
         year = 2008,
        month = dec,
       volume = {492},
       number = {2},
        pages = {401-410},
          doi = {10.1051/0004-6361:200810447},
archivePrefix = {arXiv},
       eprint = {0810.4619},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...492..401S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Patnaik2001,
       author = {{Patnaik}, A.~R. and {Narasimha}, D.},
        title = "{Determination of time delay from the gravitational lens B1422+231}",
      journal = {\mnras},
     keywords = {gravitational lensing, methods: data analysis, quasars: individual: B1422+231, Astrophysics},
         year = 2001,
        month = oct,
       volume = {326},
       number = {4},
        pages = {1403-1411},
          doi = {10.1111/j.1365-2966.2001.04711.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0106104},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.326.1403P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bonvin2019,
       author = {{Bonvin}, V. and {Millon}, M. and {Chan}, J.~H. -H. and {Courbin}, F. and {Rusu}, C.~E. and {Sluse}, D. and {Suyu}, S.~H. and {Wong}, K.~C. and {Fassnacht}, C.~D. and {Marshall}, P.~J. and {Treu}, T. and {Buckley-Geer}, E. and {Frieman}, J. and {Hempel}, A. and {Kim}, S. and {Lachaume}, R. and {Rabus}, M. and {Chao}, D.~C. -Y. and {Chijani}, M. and {Gilman}, D. and {Gilmore}, K. and {Rojas}, K. and {Williams}, P. and {Anguita}, T. and {Kochanek}, C.~S. and {Morgan}, C. and {Motta}, V. and {Tewes}, M. and {Meylan}, G.},
        title = "{COSMOGRAIL. XVIII. time delays of the quadruply lensed quasar WFI2033-4723}",
      journal = {\aap},
     keywords = {gravitational lensing: strong, galaxies: individual: WFI2033-4723, cosmological parameters, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2019,
        month = sep,
       volume = {629},
          eid = {A97},
        pages = {A97},
          doi = {10.1051/0004-6361/201935921},
archivePrefix = {arXiv},
       eprint = {1905.08260},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...629A..97B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yonehara2008,
       author = {{Yonehara}, A. and {Hirashita}, H. and {Richter}, P.},
        title = "{Origin of chromatic features in multiple quasars. Variability, dust, or microlensing}",
      journal = {\aap},
     keywords = {accretion, accretion disks, gravitational lensing, ISM:, dust, extinction, galaxies: quasars: general, Astrophysics},
         year = 2008,
        month = jan,
       volume = {478},
       number = {1},
        pages = {95-109},
          doi = {10.1051/0004-6361:20067014},
archivePrefix = {arXiv},
       eprint = {0709.1527},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...478...95Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wilhite2005,
       author = {{Wilhite}, Brian C. and {Vanden Berk}, Daniel E. and {Kron}, Richard G. and {Schneider}, Donald P. and {Pereyra}, Nicholas and {Brunner}, Robert J. and {Richards}, Gordon T. and {Brinkmann}, Jonathan V.},
        title = "{Spectral Variability of Quasars in the Sloan Digital Sky Survey. I. Wavelength Dependence}",
      journal = {\apj},
     keywords = {Galaxies: Active, Galaxies: Quasars: General, Techniques: Spectroscopic, Astrophysics},
         year = 2005,
        month = nov,
       volume = {633},
       number = {2},
        pages = {638-648},
          doi = {10.1086/430821},
archivePrefix = {arXiv},
       eprint = {astro-ph/0504309},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...633..638W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cristiani1997,
       author = {{Cristiani}, S. and {Trentini}, S. and {La Franca}, F. and {Andreani}, P.},
        title = "{The optical variability of QSOs. II. The wavelength dependence.}",
      journal = {\aap},
     keywords = {QUASARS: GENERAL, Astrophysics},
         year = 1997,
        month = may,
       volume = {321},
        pages = {123-128},
archivePrefix = {arXiv},
       eprint = {astro-ph/9610108},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997A&A...321..123C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pelt1998,
       author = {{Pelt}, J. and {Schild}, R. and {Refsdal}, S. and {Stabell}, R.},
        title = "{Microlensing on different timescales in the lightcurves of QSO 0957+561 A,B}",
      journal = {\aap},
     keywords = {METHODS: STATISTICAL, METHODS: DATA ANALYSIS, QUASARS: INDIVIDUAL: 0957+561A, B, GRAVITATIONAL LENSING},
         year = 1998,
        month = aug,
       volume = {336},
        pages = {829-839},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998A&A...336..829P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


